Hint Orchestration Using ACL2's Simplifier

This paper describes a strategy for providing hints during an ACL2 proof, implemented in a utility called use-termhint. An extra literal is added to the goal clause and simplified along with the rest of the goal until it is stable under simplification, after which the simplified literal is examined and a hint extracted from it. This simple technique supports some commonly desirable yet elusive features. It supports providing different hints to different cases of a case split, as well as binding variables so as to avoid repeating multiply referenced subterms. Since terms used in these hints are simplified in the same way as the rest of the goal, this strategy is also more robust against changes in the rewriting normal form than hints in which terms from the goal are written out explicitly.

==> eptcsdata.tex <==
\providecommand{\firstpage}{164}
\providecommand{\publicationstatus}{Shilpi Goel and Matt Kaufmann (Eds.):\\
ACL2 Theorem Prover and its Applications (ACL2-2018)\\
EPTCS 280, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.280.13}{10.4204/EPTCS.280.13}}

